Overhanging and touching waves in constant vorticity flows

We show the existence of periodic traveling waves at the free surface of a two dimensional, infinitely deep, and constant vorticity flow, under gravity, whose profiles are overhanging, including one which intersects itself to enclose a bubble of air. Numerical evidence has long suggested such overhanging and touching waves, but a rigorous proof has been elusive. Crapper's celebrated capillary waves in an irrotational flow have recently been shown to yield an exact solution to the problem for zero gravity, and our proof uses the implicit function theorem to construct nearby solutions for weak gravity.

==> preamble.tex <==
\usepackage[a4paper,margin=1in]{geometry}
\thispagestyle{empty}
\usepackage{amsmath,amssymb,amsthm}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\renewcommand\H{\mathcal H}
\newcommand\G{\mathcal G}
\newcommand\D{\mathbb D}
\newcommand\T{\mathbb T}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\abs}[2][]{#1\lvert #2 #1\rvert}
\newcommand{\n}[2][]{#1\lVert #2 #1\rVert}
\newcommand\C{\mathbb C}
\newcommand\R{\mathbb R}

% Maxima outputs truly awful TeX using \over. This line suppresses the
% resulting amsmath error
\makeatletter\let\over\@@over\makeatother 

